REBIND: Enhancing ground-state molecular conformation via force-based graph rewiring

Predicting the ground-state 3D molecular conformations from 2D molecular graphs is critical in computational chemistry due to its profound impact on molecular properties. Deep learning (DL) approaches have recently emerged as promising alternatives to computationally-heavy classical methods such as density functional theory (DFT). However, we discover that existing DL methods inadequately model inter-atomic forces, particularly for non-bonded atomic pairs, due to their naive usage of bonds and pairwise distances. Consequently, significant prediction errors occur for atoms with low degree (i.e., low coordination numbers) whose conformations are primarily influenced by non-bonded interactions. To address this, we propose REBIND, a novel framework that rewires molecular graphs by adding edges based on the Lennard-Jones potential to capture non-bonded interactions for low-degree atoms. Experimental results demonstrate that REBIND significantly outperforms state-of-the-art methods across various molecular sizes, achieving up to a 20\% reduction in prediction error.

==> figure_3d.tex <==
\begin{figure}[t!]
    \centering
    \includegraphics[width=\linewidth]{raw_figures/qualitative_analysis_3d.pdf}
    % \vskip -5pt
    \caption{
    Examples of visualizations and RMSD predictions from RDKit-ETKDG, GTMGC, and \system{} on the QM9 and GEOM-DRUGS datasets.
    }
    \label{Fig: figure_main}
    \vskip -10pt
\end{figure}


==> figure_obs.tex <==
\begin{figure}[t!]
    \centering
    % Subfigure 1
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{raw_figures/obs_rmsd.pdf} % Replace 'figure1.png' with your image file
        % \label{fig:subfig1}
    \end{subfigure}
    \hfill
    % Subfigure 2
    \begin{subfigure}[t]{0.45\textwidth}
        \centering
        \includegraphics[width=\linewidth]{raw_figures/figures/obs_mae.pdf} % Replace 'figure2.png' with your image file
    \end{subfigure}
    % \captionsetup{skip=0pt}
    \caption{Error analysis with respect to the relative atom degree on varing architectures in the QM9 dataset. (a) represents the average atom-wise RMSD while (b) shows the average atom-wise MAE for each bin of low-degree and high-degree atoms. $\Delta$ denotes the gap between the errors of the low-degree and high-degree bins.}
    \label{fig:figure_analysis}
    \vskip -10pt
\end{figure}

==> qualitative_analysis_degree.tex <==
\begin{wrapfigure}{r}{0.5\linewidth}
    \vskip -12pt
    \includegraphics[width=\linewidth]{qualitative_analysis_degree.pdf} 
    \vskip -5pt
    \caption{Atom-wise RMSD analysis with respect to the relative atom degree on \system{} and baselines. $\Delta$ denotes the gap between the errors of the low-degree and high-degree bins.}
    \label{Fig: figure_qualitative_degree}
    \vskip -15pt 
\end{wrapfigure}

==> table_gnn_ours.tex <==
\renewcommand{\arraystretch}{1.5}
  \begin{table*}[t!]
  \aboverulesep=0ex 
   \belowrulesep=0ex 
    \caption{Conformer prediction performance and percentage reduction (\%) of GNN-based backbone architectures after integration with \system{}, on the QM9 dataset.}
    \centering
    \resizebox{\textwidth}{!}{%
    \huge
    \begin{tabular}{ c | c | c c c c | c c c c }
    \toprule[2.2pt]
     \rowcolor{lightgray}\multicolumn{2}{ c |}{\fontsize{23}{23}\selectfont\textbf{Method}} & \multicolumn{4}{| c |}{\fontsize{23}{23}\selectfont Validation} &
     \multicolumn{4}{| c }{\fontsize{23}{23}\selectfont Test} \\
     \midrule[2.2pt]
     \textbf{\fontsize{23}{23}\selectfont Backbone} & \textbf{\fontsize{23}{23}\selectfont Methods} 
     & \fontsize{23}{23}\selectfont D-MAE $\downarrow$ & \fontsize{23}{23}\selectfont D-RMSE $\downarrow$ 
     & \fontsize{23}{23}\selectfont C-RMSD $\downarrow$ & \fontsize{23}{23}\selectfont E-RMSD $\downarrow$ 
     
     & \fontsize{23}{23}\selectfont D-MAE $\downarrow$ & \fontsize{23}{23}\selectfont D-RMSE $\downarrow$ 
     & \fontsize{23}{23}\selectfont C-RMSD $\downarrow$ & \fontsize{23}{23}\selectfont E-RMSD $\downarrow$ \\
     \hline
     \multirow{3}{*}{\textbf{GINE}} 
     & Vanilla &\fontsize{23}{23}\selectfont 0.605 &\fontsize{23}{23}\selectfont 0.950 & \fontsize{23}{23}\selectfont 0.865 & \fontsize{23}{23}\selectfont 1.703 & \fontsize{23}{23}\selectfont 0.606 & \fontsize{23}{23}\selectfont 0.946 & \fontsize{23}{23}\selectfont 0.867 & \fontsize{23}{23}\selectfont 1.696 \\
     &+ \system{}& \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.493} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.746} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.781} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 1.548} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.505} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.761} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.801} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 1.605} \\
     \cdashline{2-10}
     & Reduction $\uparrow$ & \fontsize{23}{23}\selectfont 18.46 & \fontsize{23}{23}\selectfont 21.47 & \fontsize{23}{23}\selectfont 9.66 & \fontsize{23}{23}\selectfont 9.10 & \fontsize{23}{23}\selectfont 16.65 & \fontsize{23}{23}\selectfont 19.55 & \fontsize{23}{23}\selectfont 7.61 & \fontsize{23}{23}\selectfont 5.36 \\
     \hline
     \multirow{3}{*}{\textbf{GATv2}} 
     & Vanilla & \fontsize{23}{23}\selectfont 0.382 & \fontsize{23}{23}\selectfont 0.695 & \fontsize{23}{23}\selectfont 0.711 & \fontsize{23}{23}\selectfont 1.371 & \fontsize{23}{23}\selectfont 0.382 & \fontsize{23}{23}\selectfont 0.690 & \fontsize{23}{23}\selectfont 0.712 & \fontsize{23}{23}\selectfont 1.358 \\
     &+ \system{}& \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.319} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.529} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.609} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 1.195} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.319} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.523} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.611} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 1.198} \\
    \cdashline{2-10}
     & Reduction $\uparrow$ & \fontsize{23}{23}\selectfont 16.60 & \fontsize{23}{23}\selectfont 23.90 & \fontsize{23}{23}\selectfont 14.36 & \fontsize{23}{23}\selectfont 12.83 & \fontsize{23}{23}\selectfont 16.62 & \fontsize{23}{23}\selectfont 24.14 & \fontsize{23}{23}\selectfont 14.14 & \fontsize{23}{23}\selectfont 11.77 \\
     \hline
     \multirow{3}{*}{\textbf{GraphGPS}} 
     & Vanilla & \fontsize{23}{23}\selectfont 0.283 & \fontsize{23}{23}\selectfont 0.500 & \fontsize{23}{23}\selectfont 0.711 & \fontsize{23}{23}\selectfont 1.371 & \fontsize{23}{23}\selectfont 0.283 & \fontsize{23}{23}\selectfont 0.499 & \fontsize{23}{23}\selectfont 0.546 & \fontsize{23}{23}\selectfont 1.064 \\
     &+ \system{}& \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.209} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.359} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.609} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 1.195} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.211} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.361} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.518} & \cellcolor{aliceblue}\textbf{\fontsize{23}{23}\selectfont 0.971} \\
     \cdashline{2-10}
     & Reduction $\uparrow$ & \fontsize{23}{23}\selectfont 26.04 & \fontsize{23}{23}\selectfont 28.14 & \fontsize{23}{23}\selectfont 14.36 & \fontsize{23}{23}\selectfont 12.83 & \fontsize{23}{23}\selectfont 25.55 & \fontsize{23}{23}\selectfont 27.58 & \fontsize{23}{23}\selectfont 5.11 & \fontsize{23}{23}\selectfont 8.74 \\
     \bottomrule[2.2pt]
    \end{tabular}}
    \label{Tab:table_gnn_ablation}
    \vskip -10pt
  \end{table*}

==> table_percentage_reduction.tex <==
\renewcommand{\arraystretch}{1.3}
\begin{table*}[t!]
\aboverulesep=0ex 
   \belowrulesep=0ex 
    \caption{Percentage reduction (in percentage) of \system{} compared to the best baseline performance on the QM9 and Molecule3D datasets.}
    \centering
    \resizebox{\textwidth}{!}{%
    \large
    \begin{tabular}{ c | c c | c c }
    \toprule[1.1pt]
     \rowcolor{lightgray}{\fontsize{12}{12}\selectfont \textbf{Splits}} & 
     \multicolumn{2}{| c |}{\fontsize{12}{12}\selectfont Validation} &
     \multicolumn{2}{| c }{\fontsize{12}{12}\selectfont Test} \\
     \midrule[1.1pt]
     \textbf{ Datasets}  
     &  Reduction (C-RMSD) $\uparrow$ 
     &  Reduction (E-RMSD) $\uparrow$ 
     &  Reduction (C-RMSD) $\uparrow$ 
     &  Reduction (E-RMSD) $\uparrow$ \\
     \hline
      \fontsize{12}{12}\selectfont \textbf{QM9} &
       \fontsize{12}{12}\selectfont 24.10 &
       \fontsize{12}{12}\selectfont 24.87 &
     
       \fontsize{12}{12}\selectfont 22.46 &
       \fontsize{12}{12}\selectfont 23.75 \\
      \hline

      \fontsize{12}{12}\selectfont \textbf{Molecule3D (random)} &
       \fontsize{12}{12}\selectfont 3.25 &
       \fontsize{12}{12}\selectfont 4.68 &
     
       \fontsize{12}{12}\selectfont 3.10 &
       \fontsize{12}{12}\selectfont 4.59 \\
      \hline

      \fontsize{12}{12}\selectfont \textbf{Molecule3D (scaffold)} &
       \fontsize{12}{12}\selectfont 5.43 &
       \fontsize{12}{12}\selectfont 9.03 &
     
       \fontsize{12}{12}\selectfont 3.03 &
       \fontsize{12}{12}\selectfont 5.18 \\
     \bottomrule[1.1pt]
    \end{tabular}}
    \label{Tab:table_reduction}
    \vskip -10pt
\end{table*}
